On building an automated responding system for app reviews: What are the characteristics of reviews and their responses?

Recent studies showed that the dialogs between app developers and app users on app stores are important to increase user satisfaction and app's overall ratings. However, the large volume of reviews and the limitation of resources discourage app developers from engaging with customers through this channel. One solution to this problem is to develop an Automated Responding System for developers to respond to app reviews in a manner that is most similar to a human response. Toward designing such system, we have conducted an empirical study of the characteristics of mobile apps' reviews and their human-written responses. We found that an app reviews can have multiple fragments at sentence level with different topics and intentions. Similarly, a response also can be divided into multiple fragments with unique intentions to answer certain parts of their review (e.g., complaints, requests, or information seeking). We have also identified several characteristics of review (rating, topics, intentions, quantitative text feature) that can be used to rank review by their priority of need for response. In addition, we identified the degree of re-usability of past responses is based on their context (single app, apps of the same category, and their common features). Last but not least, a responses can be reused in another review if some parts of it can be replaced by a placeholder that is either a named-entity or a hyperlink. Based on those findings, we discuss the implications of developing an Automated Responding System to help mobile apps' developers write the responses for users reviews more effectively.

==> eval.tex <==
\section{Evaluation}
%OK
We performed several experiments to evaluate the effectiveness of our techniques on mining and recommending exception handling patterns on Android and Java APIs. All experiments are executed on a computer 64-bit Windows 10 with Intel Core i7 3.6Ghz CPU, 8GB RAM, and 1TB HDD storage. 

\begin{table}[h]
	\centering
	\caption{Data Statistics}
	\label{table:data_collection}
	\small
	\begin{tabular}{lr}
		\toprule
        \textbf{Data Collection} & \\
        \midrule
		Number of apps                     & 4000 \\
		Number of classes                         & 13,969,235 \\
		Number of methods                         & 16,489,415 \\
		Number of bytecode instructions & 341,912,624 \\
		Space for storing .dex files				  & 19.9 GB \\
		\midrule
        \textbf{Recommending Exception Types} & \\
        \midrule
        Number of exception types                   & 261 \\
		Number of API methods                     & 64,685 \\
		Number of uncaught method sets                         & 16,489,415 \\
		Number of caught method sets                       & 549,786 \\
        \midrule
       \textbf{Recommending Repairing Methods} & \\
        \midrule
        Number of API object types                     & 360 \\
		Total number of pairs $(S_{n}, S_{h})$                         & 187,994 \\
		Average number of pairs per object type                       & 522.20 \\
        \bottomrule
	\end{tabular}
\end{table}

\subsection{Data Collection}
The dataset used in our evaluation is summarized in Table \ref{table:data_collection}. In total, we downloaded and analyzed 4000 top free apps from 36 categories in Google Play Store. To ensure the quality of training data, when crawling apps, the app extractor only downloaded apps has overall rating of at least 3 (out of 5). This filtering is based on assumption that the high-rating apps would have high quality of code, and thus, would have better exception handling mechanism. 

Since Android mobile apps are distributed as \code{.apk} files, our app extractor unpacked each \code{.apk} file and kept only its \code{.dex} file. The total storage space for the \code{.dex} files of all downloaded apps is around 19.9 GB. After parsing those \code{.dex} files we obtained about \textbf{13 millions} classes. We next developed a bytecode analyzer that analyzed each class and looked for all methods in the class to build {\groum} models. Since an Android mobile app is self-contained, its \code{.dex} file contains bytecode of all external libraries it uses. That leads to the duplication of bytecode of shared libraries. Thus, our bytecode analyzer maintains a dictionary of the analyzed methods, thus, is able to analyze each method only once. In the end, we analyzed over \textbf{16 millions} methods which have in total nearly \textbf{340 millions} bytecode instructions.

\subsection{Recommending Exception Types}
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.3\textwidth}
    	\centering
        \includegraphics[scale = 0.1]{empirical_examples/xrank}
		\caption{The accuracy of {\one}}
		\label{xrank}
    \end{minipage}
    \hfill
    \begin{minipage}{0.3\textwidth}
    	\centering
        \includegraphics[scale = 0.1]{empirical_examples/xhand}
		\caption{The accuracy of {\two}}
		\label{xhand}
    \end{minipage}
    \hfill
    \begin{minipage}{0.3\textwidth}
    	\centering
        \includegraphics[scale = 0.1]{empirical_examples/xrank2}
		\caption{The F1-score by threshold}
		\label{xrank2}
    \end{minipage}
\end{figure*}

For training and testing {\one}, the bytecode analyzer extract all caught and uncaught method sets from {\groum}. A caught method set is a set of method calls that appear in a same \code{try} block, and is associated with a catching exception. Uncaught method set is the set of all methods calls appeared in the same method implementation that are not in any \code{try } blocks. Uncaught method sets represent usages of methods that are not associate with exceptions, and vice versa.

Table \ref{table:data_collection} shows the statistics of the dataset that we extracted to evaluate {\one}. Overall, the dataset is sufficient for the evaluation. We collected over 16 millions uncaught method sets and roughly 550 thousands caught method sets. There are over 64 thousands Android API methods and total of 260 exception types. 

We evaluated the performance of {\one} on the task of recommending catching exception. Given a set of methods $S$ in the testing set, let also assume that $S$ is caught by an exception $E$ in the code, {\one} will return a rank list of exception types $R$, each exception type $r_i$ in $R$ is associated with a score represents the possibility of catching $r_i$ on $S$. To evaluate {\one}, we find the position of $E$ in $R$, if $E = r_k$ we consider it as a hit at top-$k$. We then evaluate for all caught method sets in testing sets. Finally we calculate the top-$k$ accuracy as the ratio of the total hit at $k$ over the size of testing set.

We also used 10-fold cross validation to evaluate {\one}. The dataset of apps were divided into 10 folds. At each iteration, we trained {\one} with nine folds then tested {\one} on remaining fold. Finally, we averaged the results of all iterations to produce the final top-$k$. 

To measure the effectiveness of {\one}, we compared it with a baseline method based on the frequency of catching exception types. Given a caught method set $S$, we built a lists of exception types $R$ such as each exception type $r_i \in R$ . The list $R$ is ranked based on the frequency of each exception types appeared in the training set. The assumption here is that an exception type appeared more frequent would have higher rank.

Figure \ref{xrank} shows the experiment result on recommending catching exception. From the figure we can see that both {\one} and the baseline have consistent accuracy. More importantly, {\one} recommends exception with very high levels of accuracy. For example, it has top-1 accuracy of 70\%, top-3 accuracy of 87\%. Top-5 accuracy of {\one} model approaches 94\%. In addition, {\one} significantly outperforms the baseline. For example, the corresponding top-1 and top-3 accuracy of n-gram model are 37\% (52\% lower) and 55\% (63\% lower). Overall, {\one} has a significant improvement over the baseline. The result shows that the context (method calls in \code{try} blocks) which is captured by {\one} plays an important role in the accuracy of the recommendation model.

\subsection{Recommending Repairing Method Calls}
For evaluating {\two}, the bytecode analyzer extracted all pairs $(S_{n}, S_{h})$ where $S_{n}$ is the set of method calls in \code{try} blocks and $S_{h}$ is the  repairing method call sequence in the corresponding \code{catch} block. Because {\two} is learned for each object type, thus, all method calls in both $(S_{n}, S_{h})$ belong to a same class. 

We performed an experiment to evaluate the accuracy of {\two} model in recommending repairing method call sequences. We chose the task of recommending the next repairing method call. Given the set of method calls $S_{n}$ in a \code{try} block and $i-1$ previous repairing method calls in the exception handler, the {\two} model is expected to recommend the most probable next method call at position $i$ of the exception handler. This recommendation task has been widely used in software engineering research to evaluate code completion models \cite{ngram, gralan, nguyen_salad}.

In this type of experiment, the {\two} model predicts method calls at all positions of every exception handling method sequence $S_{h}$ in the testing set. {\two} utilizes a multi-class classification model to predict the first method in the handling sequence. For a method call $c_i$ at position $i$ of $S_{h}$, we use the {\two} model to infer the top-$k$ most probable method calls $T_k = \{h_1, ..., h_k\}$. If $c_i$ is in $T_k$, we consider it as hit, i.e. an accurate top-$k$ recommendation. The top-$k$ accuracy is the ratio of the total hits over the total number of recommendations. 

All {\two} models are trained using J48 decision tree \cite{statisticallearning} and 2-gram model with Witten-Bell smoothing technique \cite{ngram, nguyen_salad}. Similar to {\one} , our experiment for {\two} is a 10-fold cross validation. We only test API object types that have more than or equals to 10 pairs of $(S_{n}, S_{h})$. As shown in the Table \ref{table:data_collection}, we performed the experiment on 360 object types. On average each object type has 522 pairs of $(S_{n}, S_{h})$.

We compared {\two} with a baseline model based on just the frequency of repairing method calls. At each position $i$, the baseline model recommends the rank list of repairing method calls based on their frequency. The method calls at previous positions are removed from the rank list when providing recommendation.
 
Figure \ref{xhand} shows the top-5 accuracy of {\two} and the baseline on recommending repairing method call sequences. From the figure we can see that {\two} recommends method calls with very high levels of accuracy. For example, it has top-1 accuracy of 89\%, top-2 accuracy of 92\%, top-3 accuracy of 96\%. Top-5 accuracy of {\two} approaches 100\%. Additionally, {\two} outperforms the baseline significantly. The baseline achieves 70\% (23\% lower) in top-1 accuracy, 83\% (11\% lower) in top-2 accuracy, and 89\% (8\% lower) in top-3 accuracy.

\subsection{Empirical Evaluation}
%We have developed {\tool} as a code recommendation tool for exception handling. {\tool} is released as a plugin of IntelliJ IDEA and Android Studio, two popular IDEs for Java programs and Android mobile apps. {\tool} predicts what types of exception could occur in a given piece of code and recommends proper exception handling code for such an exception. When requested, it will add such code into the given piece of code.
In the section, we present our evaluation on the effectiveness of {\tool} on detecting and fixing real exception bugs. 

\subsubsection{Detecting Exception Related Bugs}
With the usage described above, we can see that {\tool} could be applied to detect real exception related bugs. In particular, we focus on exception bugs. To evaluate {\tool}, we manually collected 128 exception bug fixes from the 10 open-source Android projects in our empirical dataset. Each exception bug fix is a fix for an exception bug in which developers add a \code{try-catch} block to handle exceptions.  To measure the recall in detecting exception bugs, we also collected of 128 code snippets that are very unlikely to throw any exceptions. Each code snippet appears in a project of our empirical dataset and have not be wrapped or contains any \code{try-catch} blocks. It also has not been changed and modified through the development process of the project. The code snippets are considered as \textit{negative} examples. Overall, the dataset contains 256 samples. For each sample, we use {\tool} to recommend whether or not adding a \code{try-catch} block on the code. {\tool} should recommend adding a \code{try-catch} block for an exception bug and recommend not adding any \code{try-catch} blocks on a \textit{negative} example. We then measure the accuracy of {\tool} in this task using F1-score \cite{statisticallearning}.

\begin{table}[h]
	\centering
	\sf
	\caption{Result in detecting exception bugs}
	\label{result:xrank}
	\begin{tabular}{lr}
		\toprule
		Exception bugs                    & 128            \\
		Recommended by {\tool}                & 116              \\
		Top-1 accuracy   & 86              \\
		Top-2 accuracy         & 96              \\
		Top-3 accuracy  & 104            \\
		\bottomrule
	\end{tabular}
\end{table}

Figure \ref{xrank2} shows the F1-score of {\tool} by the selection threshold used to determine whether to recommend adding a \code{try-catch} block to a sample. If the threshold is small ($5\%$ or $10\%$), {\tool} has a tendency to recommend adding exception handlers (high precision but low recall), thus, the F1-score is low. Conversely, if the threshold is big ($75\%$), {\tool} is likely to recommend not adding \code{try-catch} blocks, which also yields a low F1-score. From the figure, we can see that the F1-score yields high values in the range from $20\%$ to $50\%$ and peaks at $25\%$. Thus, we selected $25\%$ as the selection threshold to use in further evaluation of our tool.

Next, for all exception bugs detect by {\tool}, we also compared the exception types recommended by {\tool} with the one provided by developer. Overall, {\tool} achieves a high level of accuracy in predicting exception types. Over 128 exception bugs, {\tool} recommends adding exception handling blocks for 116 cases (90.62\%). It recommends the exception types in top-1 recommendation for 86 cases (74.13\%), top-2 recommendation for 96 cases (82.75\%), and top-3 for 104 cases (89.65\%).

\subsubsection{Handling Exception Bugs}
In the section, we evaluate the effectiveness of {\tool} in recommending repairing actions for real exception bug fixes. As we focus repairing actions related to Android APIs, we collected a dataset contains 42 exception bug fixes from the same 10 Android open-source projects as in the previous section. In each bug fix of the dataset, developers performed at least one repairing action (i.e. a method call, an assignment, etc.) in the exception handling code. Figure \ref{empirical:example1} in the previous section shows an example of a bug fix in the dataset. In the bug fix, the developer performed three method calls and one assignment to set value for \code{postContent}.

\begin{table}[h]
	\centering
	\caption{Result in recommending repairing actions}
	\label{second:table}
	\begin{tabular}{lrr}
		\toprule
		& ExAssist & Baseline \\
		\midrule
		The number of exception bug fixes                  & 42        &    42\\
		The number of matches  & 27        &  6    \\
		The number of partial matches & 3            &  3\\
		The number of misses        & 12          &    33\\
		\bottomrule
	\end{tabular}
\end{table}

For each bug fix in the dataset, we invoked {\tool} to recommend repairing actions and compare the recommendation result with the corresponding fix of the developer. 
%Note that, as a recommendation tool, we has improved the functionality of {\tool} by not only recommending repairing method calls but also recommending other actions such as assigning a default value for a variable, returning a default value, etc. 
If the recovery actions recommended by {\tool} exactly match with the fix, we count it as a match. If the recommended actions of {\tool} contain the code in the fix of the developer, we count it as a partial match. Otherwise, we consider the case as a miss. 

To further evaluate the effectiveness of {\tool}, we compare our tool with a well known existing
approach provided by Barbosa \textit{et al.} \cite{barbosa_heuristic}. In their work, they proposed three heuristic strategies used to recommend exception handling code in programming tasks. We re-implemented the technique using the same configurations presented in the work. 

Table \ref{second:table} shows the evaluation result of {\tool} and the baseline for the task. In the total of 42 exception bug fixes, the recommendations of {\tool} match the fixes of developers in 27 cases. There are 3 cases in which the recommended actions of {\tool} contain the fix code. Overall, {\tool} could provide meaningful recommendations in roughly 64\% of the bug fixes. 








